SeriesBench: A Benchmark for Narrative-Driven Drama Series Understanding

With the rapid development of Multi-modal Large Language Models (MLLMs), an increasing number of benchmarks have been established to evaluate the video understanding capabilities of these models. However, these benchmarks focus on standalone videos and mainly assess "visual elements" like human actions and object states. In reality, contemporary videos often encompass complex and continuous narratives, typically presented as a series. To address this challenge, we propose SeriesBench, a benchmark consisting of 105 carefully curated narrative-driven series, covering 28 specialized tasks that require deep narrative understanding. Specifically, we first select a diverse set of drama series spanning various genres. Then, we introduce a novel long-span narrative annotation method, combined with a full-information transformation approach to convert manual annotations into diverse task formats. To further enhance model capacity for detailed analysis of plot structures and character relationships within series, we propose a novel narrative reasoning framework, PC-DCoT. Extensive results on SeriesBench indicate that existing MLLMs still face significant challenges in understanding narrative-driven series, while PC-DCoT enables these MLLMs to achieve performance improvements. Overall, our SeriesBench and PC-DCoT highlight the critical necessity of advancing model capabilities to understand narrative-driven series, guiding the future development of MLLMs. SeriesBench is publicly available at https://github.com/zackhxn/SeriesBench-CVPR2025.

==> table/clip_cnclip.tex <==
\begin{table}[!ht]
    \centering
    \vspace{-10pt}
    \small
    \renewcommand\tabcolsep{8pt} % column space
    \renewcommand\arraystretch{0.85} % row space
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|l}
            \toprule
            \multicolumn{1}{c|}{\textbf{Model}}
         
            % & \makecell{\textbf{LLM} \\ \textbf{Params}}
       
            & \textbf{VS}
            & \textbf{SC}
            & \textbf{AU}
            & \textbf{AG}
            & \textbf{CO}
            & \multicolumn{1}{c}{\textbf{Overall}} \\
            \midrule
            Qwen2-VL+PC-DCoT$_{\text{custom-CLIP}}$   
            & 75.2 & 73.5 & 69.7 & 80.9 & 67.4 &\textbf{73.9} \\
            Qwen2-VL+PC-DCoT$_{\text{CN-CLIP}}$
            & 73.6 & 71.8 & 68.6 & 79.7 & 65.8 & \textbf{72.4}{\footnotesize (\textit{{$\downarrow$}1.5})}  \\
            \bottomrule
        \end{tabular}
    }
    
    \vspace{-0.35cm} % 调整间距，负值表示减少间距

    \label{tab:lora}
\end{table}


==> table/compare_rebuttal.tex <==
\begin{table}[!ht]
\centering

\vspace{-10pt}
\label{T:main}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{0.6} % 调小行间距（默认值为1）
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\multirow{3}{*}{Benchmark} & \multirow{3}{*}{Series}& \multicolumn{5}{c}{Dimension} & \multirow{3}{*}{Sub.Tokens} & \multirow{3}{*}{Anno.} & \multicolumn{2}{c}{Video}  & \multirow{3}{*}{Multi Tasks}    \\
\cmidrule(lr){3-7} \cmidrule(lr){10-11}  
 & & VS & SC & AU & AG & CO & & & \#Clips & Len.   \\
 \toprule

MoviePuzzle & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \includegraphics[width=0.02\textwidth]{figures/human.png}&  10031 & - & \textcolor{darkred}{\ding{55}} \\
% ~\cite{wang2023moviepuzzle}

LongVideoBench & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \includegraphics[width=0.02\textwidth]{figures/human.png}&  3763 & 473.0 & \textcolor{darkred}{\ding{55}} \\
% ~\cite{wu2024longvideobench}
\midrule
\textbf{SeriesBench (Ours)} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textbf{250.2} &  \includegraphics[width=0.02\textwidth]{figures/human.png} & 1072 & 79.2 &\textcolor{darkgreen}{\ding{51}} \\


\bottomrule 

\end{tabular}}
\vspace{-0.6cm}
\label{tab:compare_rebuttal}
\end{table}

==> table/lora_merge.tex <==
\begin{table}[!ht]
    \centering
    \vspace{-10pt}
    \small
    \renewcommand\tabcolsep{8pt} % column space
    \renewcommand\arraystretch{0.85} % row space
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|l}
            \toprule
            \multicolumn{1}{c|}{\textbf{Model}}
         
            % & \makecell{\textbf{LLM} \\ \textbf{Params}}
       
            & \textbf{VS}
            & \textbf{SC}
            & \textbf{AU}
            & \textbf{AG}
            & \textbf{CO}
            & \multicolumn{1}{c}{\textbf{Overall}} \\
            \midrule
            Qwen2-VL          
            & 55.7 & 57.5 & 58.6 & 75.3 & 59.6 & \textbf{60.3} \\
            \hspace{6mm}+Lora
            & 66.9 & 65.4 & 68.7 & 82.5 & 67.6 & \textbf{68.2}{\footnotesize (\textit{{$\uparrow$}7.9})}  \\
            \hspace{6mm}+Lora+PC-DCoT
            & 78.1 & 76.8 & 72.3 & 84.4 & 71.7 & \textbf{77.1}{\footnotesize (\textit{{$\uparrow$}16.8})}  \\
            \bottomrule
        \end{tabular}
    }
    \vspace{-0.5cm} % 调整间距，负值表示减少间距
    \label{tab:lora}
\end{table}


==> table/vita_audio.tex <==
\begin{table}[!ht]
    \centering
    \vspace{-18pt}
    \small
    \renewcommand\tabcolsep{8pt} % column space
    \renewcommand\arraystretch{0.6} % row space
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|l}
            \toprule
            \multicolumn{1}{c|}{\textbf{Model}}
            % & \makecell{\textbf{LLM} \\ \textbf{Params}}
       
            & \textbf{VS}
            & \textbf{SC}
            & \textbf{AU}
            & \textbf{AG}
            & \textbf{CO}
            & \multicolumn{1}{c}{\textbf{Overall}} \\
            \midrule

            VITA
            & 41.6 & 44.1 & 47.2 & 59.9 & 42.9 & \textbf{46.5}  \\
            \hspace{4mm} +audio
            & 33.6 & 32.3 & 39.4 & 52.5 & 43.6 & \textbf{38.5}{\footnotesize (\textit{{$\downarrow$}8.0})}  \\
            \hspace{4mm} +sub
            & 46.9 & 46.0 & 53.3 & 68.9 & 48.1 & \textbf{51.8}{\footnotesize (\textit{{$\uparrow$}5.3})}  \\
            \hspace{4mm} +sub+audio
            & 34.1 & 30.7 & 36.0 & 61.5 & 36.5 & \textbf{38.4}{\footnotesize (\textit{{$\downarrow$}8.1})}  \\
            \bottomrule
        \end{tabular}
    }
    % \vspace{-5pt}

    \vspace{-0.5cm} % 调整间距，负值表示减少间距
    \label{tab:lora}
\end{table}

